Learning to Detect Objects from Multi-Agent LiDAR Scans without Manual Labels

Unsupervised 3D object detection serves as an important solution for offline 3D object annotation. However, due to the data sparsity and limited views, the clustering-based label fitting in unsupervised object detection often generates low-quality pseudo-labels. Multi-agent collaborative dataset, which involves the sharing of complementary observations among agents, holds the potential to break through this bottleneck. In this paper, we introduce a novel unsupervised method that learns to Detect Objects from Multi-Agent LiDAR scans, termed DOtA, without using labels from external. DOtA first uses the internally shared ego-pose and ego-shape of collaborative agents to initialize the detector, leveraging the generalization performance of neural networks to infer preliminary labels. Subsequently,DOtA uses the complementary observations between agents to perform multi-scale encoding on preliminary labels, then decodes high-quality and low-quality labels. These labels are further used as prompts to guide a correct feature learning process, thereby enhancing the performance of the unsupervised object detection task. Extensive experiments on the V2V4Real and OPV2V datasets show that our DOtA outperforms state-of-the-art unsupervised 3D object detection methods. Additionally, we also validate the effectiveness of the DOtA labels under various collaborative perception frameworks.The code is available at https://github.com/xmuqimingxia/DOtA.

==> figText/com_weakly.tex <==
\begin{table}[htbp]
	\centering
    \resizebox{0.49\textwidth}{!}{
	\begin{tabular}{c|c|ccc}
\hline 
\multirow{2}{*}{Data}     & \multirow{2}{*}{Method} & \multicolumn{3}{c}{Car-3D Detection}                            \\ \cline{3-5} 
                          &                         & \multicolumn{1}{c|}{Easy}  & \multicolumn{1}{c|}{Mod.}  & Hard  \\ \hline \hline
weakly* + 534 precisely\# & WS3D \cite{WS3D}                   & \multicolumn{1}{c|}{84.0} & \multicolumn{1}{c|}{75.1} & 73.2 \\ \hline
weakly* + 2\%Fully        & WSS3D \cite{WSS3D}                  & \multicolumn{1}{c|}{84.5}  & \multicolumn{1}{c|}{75.8}  & 71.1  \\ \hline
2\%Fully                  & Our HINTED                    & \multicolumn{1}{c|}{\textbf{90.6}}  & \multicolumn{1}{c|}{\textbf{80.4}}  & \textbf{77.6}  \\ \hline
\end{tabular}
}
\caption{Comparison with state-of-the-art weakly-supervised methods on KITTI $val$ split. *: point annotations. \#: high-quality annotated instance.}
    \label{tab:com_weak}
\end{table}

==> figText/compare-dif-distance.tex <==
\begin{figure*}[t]
  \centering
   \includegraphics[width=0.99\linewidth]{figures/diff_dist_final.pdf}
   \caption{Comparison of three categories at different thresholds. The red bars represent the performance of our HINTED, while the blue bars represent the performance of CoIn~\cite{CoIn}. N/A indicates that there are no samples at this difficulty level. }
   \label{fig:distance}
\end{figure*}


==> figText/compare-to-semi.tex <==
\begin{table*}[htbp]
	\centering
     \resizebox{0.95\textwidth}{!}{
	\begin{tabular}{c|c|c|cccc|cccc}
\hline
                                  &                                      &                               & \multicolumn{4}{c|}{1\%}                                                                                                                                                 & \multicolumn{4}{c}{2\%}                                                                                                                                                                  \\ \cline{4-11} 
\multirow{-2}{*}{Setting}         & \multirow{-2}{*}{Method}             & \multirow{-2}{*}{Modality}    & \multicolumn{1}{c|}{Car}                      & \multicolumn{1}{c|}{Ped.}                     & \multicolumn{1}{c|}{Cyc.}                     & Avg.                     & \multicolumn{1}{c|}{Car}                          & \multicolumn{1}{c|}{Ped.}                         & \multicolumn{1}{c|}{Cyc.}                         & Avg.                         \\ \hline \hline
                                  & PV-RCNN \cite{PV-RCNN}                             & LIDAR                         & \multicolumn{1}{c|}{73.5}                     & \multicolumn{1}{c|}{28.7}                     & \multicolumn{1}{c|}{28.4}                     & 43.5                     & \multicolumn{1}{c|}{76.6}                         & \multicolumn{1}{c|}{40.8}                         & \multicolumn{1}{c|}{45.5}                         & 54.3                         \\ \cline{2-11} 
                                  & 3DIoUMatch \cite{3DIoUMatch}                          & LIDAR                         & \multicolumn{1}{c|}{76.0}                     & \multicolumn{1}{c|}{31.7}                     & \multicolumn{1}{c|}{36.4}                     & 48.0                     & \multicolumn{1}{c|}{78.7}                         & \multicolumn{1}{c|}{48.2}                         & \multicolumn{1}{c|}{56.2}                         & 61.0                         \\ \cline{2-11} 
                                  & DetMatch       \cite{detmatch}                      & LIDAR+RGB                     & \multicolumn{1}{c|}{77.5}                     & \multicolumn{1}{c|}{\textbf{57.3}}                     & \multicolumn{1}{c|}{42.3}                     & 59.0                     & \multicolumn{1}{c|}{78.2}                         & \multicolumn{1}{c|}{54.1}                         & \multicolumn{1}{c|}{64.7}                         & 65.6                         \\ \cline{2-11} 
                                  & HSSDA       \cite{hssda}                         & LIDAR                         & \multicolumn{1}{c|}{\textbf{80.9}}                     & \multicolumn{1}{c|}{51.9}                     & \multicolumn{1}{c|}{45.7}                     & 59.5                     & \multicolumn{1}{c|}{\textbf{81.9}}                         & \multicolumn{1}{c|}{58.2}                         & \multicolumn{1}{c|}{65.8}                         & 68.6                         \\ \cline{2-11} 
\multirow{-5}{*}{Semi-supervised} & \cellcolor[HTML]{EFEFEF} Our HINTED & \cellcolor[HTML]{EFEFEF}LIDAR & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}79.9} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}52.1} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{50.5}} & \cellcolor[HTML]{EFEFEF}\textbf{60.5} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}80.4} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{58.9}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{73.2}} & \cellcolor[HTML]{EFEFEF}\textbf{70.8} \\ \hline
\end{tabular}
    }
    \caption{Comparison with state-of-the-art semi-supervised methods on KITTI $val$ split. All methods are built upon PV-RCNN and trained on randomly selected 2\% or 1\% fully annotated frames from $train$ split.}
    \label{tab:com_semi}
\end{table*}




==> figText/dif_fusion.tex <==
\begin{table}[htbp]
	\centering
    %\resizebox{\textwidth}{!}{
	\begin{tabular}{l||ccc}
\hline
{\color[HTML]{333333} }                                  & \multicolumn{3}{c}{{\color[HTML]{333333} Car-3D Detectin}} \\ \cline{2-4} 
\multirow{-2}{*}{{\color[HTML]{333333} Fusion Strategy}} & Easy               & Mod               & Hard              \\ \hline
\hline
Baseline                                                 & 92.0               & 79.7              & 74.2              \\
ROI-based Fusion                                         & 87.9               & 77.4              & 72.7              \\
Average-based Fusion                                     & 91.2               & 80.3              & 73.5              \\
Attension-basd Fusion                                    & \textbf{94.2}      & \textbf{82.3}     & \textbf{78.5}     \\ \hline
\end{tabular}
    %}
    \caption{The influence of different feature fusion approaches. }
    \label{tab:dif_fusion}
\end{table}




==> figText/full_compare.tex <==
\begin{table*}[htbp]
	\centering
    \resizebox{0.9\textwidth}{!}{
	\begin{tabular}{c|c|c|ccc|ccc}
\hline
                                  &                                &                                                    & \multicolumn{3}{c|}{\textbf{Car-3D  AP(R40)}}                                                                                              & \multicolumn{3}{c}{\textbf{Car-BEV  AP(R40)}}                                                                                              \\ \cline{4-9} 
\multirow{-2}{*}{Annotation Rate}            & \multirow{-2}{*}{Stage}        & \multirow{-2}{*}{Method}                           & \multicolumn{1}{c|}{Easy}                           & \multicolumn{1}{c|}{Mod}                            & Hard                           & \multicolumn{1}{c|}{Easy}                           & \multicolumn{1}{c|}{Mod}                            & Hard                           \\ \hline
100\%                             &                                & 1.CenterPoint*~\cite{CenterPoint}                                & \multicolumn{1}{c|}{89.07}                          & \multicolumn{1}{c|}{80.50}                          & 76.49                          & \multicolumn{1}{c|}{92.98}                          & \multicolumn{1}{c|}{89.01}                          & 87.50                          \\
2\%                               &                                & 2.CenterPoint~\cite{CenterPoint}                                & \multicolumn{1}{c|}{49.69}                          & \multicolumn{1}{c|}{31.55}                          & 25.91                          & \multicolumn{1}{c|}{56.78}                          & \multicolumn{1}{c|}{42.50}                          & 34.14                          \\
2\%                               &                                & 3.CoIn(Our CenterPoint-based)                          & \multicolumn{1}{c|}{72.03}                          & \multicolumn{1}{c|}{54.82}                          & 43.77                          & \multicolumn{1}{c|}{87.20}                          & \multicolumn{1}{c|}{73.54}                          & 72.03                          \\
2\%                               &                                & 4. CoIn++(Our CenterPoint-based)                    & \multicolumn{1}{c|}{\textbf{88.51}}                 & \multicolumn{1}{c|}{\textbf{75.23}}                 & \textbf{64.83}                 & \multicolumn{1}{c|}{\textbf{95.79}}                 & \multicolumn{1}{c|}{\textbf{88.10}}                 & \textbf{77.39}                 \\
\cellcolor[HTML]{FFFFFF}\textit{} &                                & \cellcolor[HTML]{DBEEF4}\textit{Improvement (3-2)} & \multicolumn{1}{c|}{\cellcolor[HTML]{DBEEF4}+22.34} & \multicolumn{1}{c|}{\cellcolor[HTML]{DBEEF4}+23.27} & \cellcolor[HTML]{DBEEF4}+17.86 & \multicolumn{1}{c|}{\cellcolor[HTML]{DBEEF4}+30.42} & \multicolumn{1}{c|}{\cellcolor[HTML]{DBEEF4}+31.04} & \cellcolor[HTML]{DBEEF4}+37.89 \\
\cellcolor[HTML]{FFFFFF}\textit{} & \multirow{-6}{*}{Single-stage} & \cellcolor[HTML]{DBEEF4}\textit{Improvement (4-1)} & \multicolumn{1}{c|}{\cellcolor[HTML]{DBEEF4}-0.56}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DBEEF4}-5.27}  & \cellcolor[HTML]{DBEEF4}-11.66 & \multicolumn{1}{c|}{\cellcolor[HTML]{DBEEF4}+2.81}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DBEEF4}-0.91}  & \cellcolor[HTML]{DBEEF4}-10.11 \\ \hline
100\%                             &                                & 1.Voxel-RCNN~\cite{Voxel-RCNN}                                 & \multicolumn{1}{c|}{92.38}                          & \multicolumn{1}{c|}{85.29}                          & 82.86                          & \multicolumn{1}{c|}{95.52}                          & \multicolumn{1}{c|}{91.25}                          & 88.99                          \\
2\%                               &                                & 2.Voxel-RCNN~\cite{Voxel-RCNN}                                 & \multicolumn{1}{c|}{70.52}                          & \multicolumn{1}{c|}{54.97}                          & 44.82                          & \multicolumn{1}{c|}{83.67}                          & \multicolumn{1}{c|}{71.14}                          & 57.71                          \\
2\%                               &                                & 3.CoIn(Our Voxel-RCNN-based)                           & \multicolumn{1}{c|}{84.56}                          & \multicolumn{1}{c|}{68.47}                          & 58.02                          & \multicolumn{1}{c|}{92.31}                          & \multicolumn{1}{c|}{81.01}                          & 70.24                          \\
2\%                               &                                & 4. CoIn++(Our Voxel-RCNN-based)                     & \multicolumn{1}{c|}{\textbf{92.01}}                 & \multicolumn{1}{c|}{\textbf{79.59}}                 & \textbf{71.58}                 & \multicolumn{1}{c|}{\textbf{96.12}}                 & \multicolumn{1}{c|}{\textbf{88.87}}                 & \textbf{82.57}                 \\
\cellcolor[HTML]{FFFFFF}\textit{} &                                & \cellcolor[HTML]{DBEEF4}\textit{Improvement (3-2)} & \multicolumn{1}{c|}{\cellcolor[HTML]{DBEEF4}+14.04} & \multicolumn{1}{c|}{\cellcolor[HTML]{DBEEF4}+13.5}  & \cellcolor[HTML]{DBEEF4}+13.2  & \multicolumn{1}{c|}{\cellcolor[HTML]{DBEEF4}+8.64}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DBEEF4}+9.87}  & \cellcolor[HTML]{DBEEF4}+12.53 \\
\cellcolor[HTML]{FFFFFF}\textit{} & \multirow{-6}{*}{Two-stage}    & \cellcolor[HTML]{DBEEF4}\textit{Improvement (4-1)} & \multicolumn{1}{c|}{\cellcolor[HTML]{DBEEF4}-0.37}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DBEEF4}-5.7}   & \cellcolor[HTML]{DBEEF4}-11.28 & \multicolumn{1}{c|}{\cellcolor[HTML]{DBEEF4}+0.6}   & \multicolumn{1}{c|}{\cellcolor[HTML]{DBEEF4}-2.38}  & \cellcolor[HTML]{DBEEF4}-6.42  \\ \hline
100\%                             &                                & 1.CasA~\cite{CasA}                                       & \multicolumn{1}{c|}{93.08}                          & \multicolumn{1}{c|}{86.33}                          & 81.86                          & \multicolumn{1}{c|}{93.93}                          & \multicolumn{1}{c|}{90.20}                          & 87.72                          \\
2\%                               &                                & 2.CasA~\cite{CasA}                                         & \multicolumn{1}{c|}{74.18}                          & \multicolumn{1}{c|}{57.37}                          & 45.05                          & \multicolumn{1}{c|}{85.90}                          & \multicolumn{1}{c|}{73.21}                          & 57.23                          \\
2\%                               &                                & 3.CoIn(Our CasA-based)                                 & \multicolumn{1}{c|}{89.17}                          & \multicolumn{1}{c|}{75.32}                          & 62.98                          & \multicolumn{1}{c|}{95.99}                          & \multicolumn{1}{c|}{85.02}                          & 72.47                          \\
2\%                               &                                & 4. CoIn++( Our CasA-based)                           & \multicolumn{1}{c|}{\textbf{93.08}}                 & \multicolumn{1}{c|}{\textbf{82.80}}                 & \textbf{74.67}                 & \multicolumn{1}{c|}{\textbf{96.82}}                 & \multicolumn{1}{c|}{\textbf{91.31}}                 & \textbf{84.00}                 \\
\cellcolor[HTML]{FFFFFF}\textit{} &                                & \cellcolor[HTML]{DBEEF4}\textit{Improvement (3-2)} & \multicolumn{1}{c|}{\cellcolor[HTML]{DBEEF4}+14.99} & \multicolumn{1}{c|}{\cellcolor[HTML]{DBEEF4}+17.95} & \cellcolor[HTML]{DBEEF4}+17.93 & \multicolumn{1}{c|}{\cellcolor[HTML]{DBEEF4}+10.09} & \multicolumn{1}{c|}{\cellcolor[HTML]{DBEEF4}+11.81} & \cellcolor[HTML]{DBEEF4}+15.24 \\
\cellcolor[HTML]{FFFFFF}\textit{} & \multirow{-6}{*}{Multi-stage}  & \cellcolor[HTML]{DBEEF4}\textit{Improvement (4-1)} & \multicolumn{1}{c|}{\cellcolor[HTML]{DBEEF4}0}      & \multicolumn{1}{c|}{\cellcolor[HTML]{DBEEF4}-3.53}  & \cellcolor[HTML]{DBEEF4}-7.19  & \multicolumn{1}{c|}{\cellcolor[HTML]{DBEEF4}+2.89}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DBEEF4}+1.11}  & \cellcolor[HTML]{DBEEF4}-3.72  \\ \hline
\end{tabular}
    }
    \caption{Comparison with different detectors with full annotations (100\%) and extremely limited annotations (2\%) on KITTI $val$ split. The 3D object detection benchmark is evaluated by mean average percision with R40, under IoU thresholds 0.7. * denotes the results obtained by referring to its open source code. ++ indicates the addition of instance-level pseudo-label mining methods referring to SS3D~\cite{ss3d}. }
    \label{tab:full_compare}
\end{table*}

==> figText/introduction_motivation.tex <==
\begin{figure}[t]
  \centering
   \includegraphics[width=1\linewidth]{figures/dif_rate_perfomance.pdf}
   \caption{Comparison of performance with different annotation rates under the KITTI-3D-Car benchmark. Green and orange represent CenterPoint\cite{CenterPoint} and our proposed CoIn, respectively.
   }
   \label{fig:motivation}
\end{figure}

==> figText/introduction_performance.tex <==
\begin{figure}[t]
  \centering
   \includegraphics[width=1\linewidth]{figures/performance.pdf}
   \caption{Our VirConv-T achieves top average precision (AP) on both 3D and BEV moderate car detection in the KITTI benchmark. Our VirConv-L runs fast at 56ms with competitive AP.}
   \label{fig:performance}
\end{figure}

==> figText/kitti_dif_sample_rate.tex <==
\begin{table}[htbp]
	\centering
    %\resizebox{\textwidth}{!}{
	\begin{tabular}{c||c||ccc}
\hline
\multirow{2}{*}{Sampling method} & \multirow{2}{*}{ratio} & \multicolumn{3}{c}{Car-3D Detection}                                                                 \\ \cline{3-5} 
                                 &                        & \multicolumn{1}{c|}{Easy}           & \multicolumn{1}{c|}{Mod.}           & Hard           \\ \hline \hline
\multirow{3}{*}{FPS}             & 40\%                   & \multicolumn{1}{c|}{93.89}      & \multicolumn{1}{c|}{81.67}      & 76.21      \\
                                 & 20\%                   & \multicolumn{1}{c|}{94.09}          & \multicolumn{1}{c|}{81.71}          & 76.48          \\
                                 & 10\%                   & \multicolumn{1}{c|}{93.97}      & \multicolumn{1}{c|}{81.59}      & 76.23      \\ \hline \hline
\multirow{3}{*}{RS}              & 40\%                   & \multicolumn{1}{c|}{94.26}          & \multicolumn{1}{c|}{81.66}          & 76.19          \\
                                 & 20\%                   & \multicolumn{1}{c|}{\textbf{94.33}} & \multicolumn{1}{c|}{\textbf{82.56}} & \textbf{78.75} \\
                                 & 10\%                   & \multicolumn{1}{c|}{94.25}          & \multicolumn{1}{c|}{82.34}          & 78.51          \\ \hline
\end{tabular}
    %}
    \caption{Comparison of different sample strategies on KITTI $val$ split. 
    %For each sampling strategy, 
    %we report 3D detection results in three sampling rates. %(40\%, 20\%, 10\%).
    }
    \label{tab:kitti_dif_sample_rate}
\end{table}




==> figText/method_matri_multi.tex <==
\begin{figure}[t]
  \centering
   \includegraphics[width=1\linewidth]{figures/matric_multipul.pdf}
   \caption{Illustration of similarity matrix computing processing. Let $K=N=3$ to understand the meaning of matrix. 
}
   \label{fig:matrix}
\end{figure}


==> figText/method_mmcont.tex <==
\begin{figure}[t]
  \centering
   \includegraphics[width=0.9\linewidth]{figures/MMcont.pdf}
   \caption{Feature space. Left: indistinguishab feature space; Right: discriminative feature space.
}
   \label{fig:mmcont}
\end{figure}


==> figText/val_waymo.tex <==
\begin{table*}[htbp]
	\centering
	\small
    %\resizebox{\columnwidth}{!}{
	\begin{tabular}{c|c|cc|cc|cc}
\hline
                                      &                                               & \multicolumn{2}{c|}{VEHICLE}                                                  & \multicolumn{2}{c|}{PEDESTRIAN}                                           & \multicolumn{2}{c}{CYCLIST}                                               \\ \cline{3-8} 
                                      &                                               & LEVEL\_1                              & LEVEL\_2                              & LEVEL\_1                            & LEVEL\_2                            & LEVEL\_1                            & LEVEL\_2                            \\ \cline{3-8} 
\multirow{-3}{*}{Data}                & \multirow{-3}{*}{Method}                      & AP/APH                                & AP/APH                                & AP/APH                              & AP/APH                              & AP/APH                              & AP/APH                              \\ \hline
Full-supervised                       & CentePoint                                    & 67.00/66.41                           & 59.14/58.61                           & 69.51/62.87                         & 61.62/55.59                         & 67.83/66.39                         & 65.32/63.94                         \\ \hline
                                      & CentePoint                                    & 32.15/31.55                           & 27.97/27.45                           & 25.66/21.65                         & 22.00/18.56                         & 59.25/57.84                         & 57.22/55.86                         \\
                                      & CoIn                                          & 48.25/47.60                           & 41.82/41.25                           & 28.25/24.28                         & 23.79/20.45                         & 63.99/62.60                         & 61.71/60.37                         \\
\multirow{-3}{*}{Sparsely-supervised} & \cellcolor[HTML]{DBEEF4}\textit{Improvements} & \cellcolor[HTML]{DBEEF4}+16.10/+16.05 & \cellcolor[HTML]{DBEEF4}+13.85/+13.80 & \cellcolor[HTML]{DBEEF4}+2.59/+2.63 & \cellcolor[HTML]{DBEEF4}+1.79/+1.89 & \cellcolor[HTML]{DBEEF4}+4.74/+4.76 & \cellcolor[HTML]{DBEEF4}+4.49/+4.51 \\ \hline
\end{tabular}
    %}
    \caption{Comparison on the Waymo open dataset for vehicle detection, pedestrian detection, and cyclist detection.}
    \label{tab:val_waymo}
\end{table*}

==> text/limitation.tex <==
 \section{Limitation}


 %yuxunlianmoxing，训练时间长

Due to limited memory, we cannot parallelize the generation of feature maps in the student network using shared weights, leading to longer training times. Additionally, we have only experimented with the basic architecture of VoxelRCNN, and its effectiveness with more advanced frameworks will be further validated in future work.
